Iterative Refinement of Project-Level Code Context for Precise Code Generation with Compiler Feedback

Large Language Models (LLMs) have shown remarkable progress in automated code generation. Yet, LLM-generated code may contain errors in API usage, class, data structure, or missing project-specific information. As much of this project-specific context cannot fit into the prompts of LLMs, we must find ways to allow the model to explore the project-level code context. We present CoCoGen, a new code generation approach that uses compiler feedback to improve the LLM-generated code. CoCoGen first leverages static analysis to identify mismatches between the generated code and the project's context. It then iteratively aligns and fixes the identified errors using information extracted from the code repository. We integrate CoCoGen with two representative LLMs, i.e., GPT-3.5-Turbo and Code Llama (13B), and apply it to Python code generation. Experimental results show that CoCoGen significantly improves the vanilla LLMs by over 80% in generating code dependent on the project context and consistently outperforms the existing retrieval-based code generation baselines.

==> tables/4_dataset_statistic.tex <==
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{c}{\textbf{Dependency Type}} & \multicolumn{1}{c}{\textbf{NS}} & \multicolumn{1}{c}{\textbf{API}} & \multicolumn{1}{c}{\textbf{Class}} & \textbf{Vars} & \textbf{Q.} & \textbf{S.} \\ \hline
\multicolumn{7}{l}{\textit{Function-level}}                                                                                                                                             \\
Self-contained                      & $35$                              & $0.0$                              & $0.0$                                & $0.0$           & $47.1$        & $203.8$       \\
Slib-runnable                      & $28$                              & $3.2$                              & $1.8$                                & $1.4$           & $59.7$        & $269.4$       \\
Plib-runnable                      & $21$                              & $4.1$                              & $2.0$                                & $1.8$          & $40.2$        & $332.0$       \\ \hline
\multicolumn{7}{l}{\textit{Project-level}}                                                                                                                                             \\
Class-runnable                        & $55$                              & $4.4$                              & $1.1$                                & $3.3$           & $50.6$        & $544.1$       \\
File-runnable                        & $68$                              & $4.8$                              & $1.5$                                & $2.2$           & $41.4$        & $771.3$       \\
Project-runnable                        & $23$                              & $6.0$                              & $3.8$                                & $2.8$           & $95.9$        & $733.5$       \\ \hline
\end{tabular}

==> tables/5.5_ablation_large_rebuttal.tex <==
\begin{tabular}{lccccccccccc}
\hline
Data Split            & \multicolumn{3}{c}{\textbf{Class Runnable}}                                                                                                & \multicolumn{1}{l}{\textbf{}}                & \multicolumn{3}{c}{\textbf{File Runnable}}                                                                                                 & \multicolumn{1}{l}{}                         & \multicolumn{3}{c}{\textbf{Project Runnable}}                                                                                              \\ \cline{1-4} \cline{6-8} \cline{10-12} 
Method                & Pass@1                                       & Pass@5                                       & Pass@10                                      &                                              & Pass@1                                       & Pass@5                                       & Pass@10                                      &                                              & Pass@1                                       & Pass@5                                       & Pass@10                                      \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{4}{l}{\cellcolor[HTML]{EFEFEF}LLM: GPT-3.5-Turbo}                                                                                                     & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} \\
Direct                & 8.73                                         & 12.57                                        & 14.55                                        &                                              & 19.85                                        & 27.62                                        & 30.88                                        &                                              & 9.57                                         & 12.08                                        & 13.04                                        \\
\rowcolor[HTML]{EFEFEF} 
ReACC                 & 20.36                                        & 33.27                                        & 38.18                                        &                                              & 17.65                                        & 28.92                                        & 33.82                                        &                                              & 11.30                                        & 19.53                                        & 21.74                                        \\
RepoCoder             & \textbf{35.45}                               & 40.46                                        & 41.82                                        &                                              & 29.41                                        & 34.61                                        & 36.76                                        &                                              & 16.96                                        & 19.57                                        & 21.74                                        \\
\rowcolor[HTML]{EFEFEF} 
\tool                 & 28.00                                        & 44.92                                        & \textbf{49.09}                               &                                              & \textbf{30.29}                               & \textbf{43.58}                               & \textbf{47.06}                               &                                              & \textbf{21.30}                               & \textbf{36.73}                               & \textbf{39.13}                               \\
w/ CF                 & 30.00                                        & 42.58                                        & 45.45                                        &                                              & 26.03                                        & 37.41                                        & 42.65                                        &                                              & 14.35                                        & 25.62                                        & 30.43                                        \\
\rowcolor[HTML]{EFEFEF} 
w/ CF+SQL             & 30.36                                        & 44.61                                        & 49.09                                        &                                              & 26.76                                        & 37.68                                        & 39.71                                        &                                              & 15.65                                        & 25.12                                        & 30.43                                        \\
w/ CF+Semantic        & \textbf{31.45}                               & \textbf{45.00}                               & 47.27                                        &                                              & 27.35                                        & 39.90                                        & 45.45                                        &                                              & 17.83                                        & 28.50                                        & 34.78                                        \\ \hline
\rowcolor[HTML]{EFEFEF} 
LLM: Code Llama (13B) & \multicolumn{1}{r}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{r}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{r}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} \\
Direct                & 18.91                                        & 30.65                                        & 34.55                                        &                                              & 18.53                                        & 27.82                                        & 29.41                                        &                                              & 5.22                                         & 8.70                                         & 13.04                                        \\
\rowcolor[HTML]{EFEFEF} 
ReACC                 & 20.36                                        & 33.27                                        & 38.18                                        &                                              & \textbf{17.65}                               & 27.61                                        & 33.82                                        &                                              & 11.30                                        & 19.53                                        & 21.74                                        \\
RepoCoder             & 17.82                                        & 35.22                                        & 40.00                                        &                                              & 15.00                                        & 28.31                                        & 32.35                                        &                                              & \textbf{16.09}                               & 21.36                                        & 21.74                                        \\
\rowcolor[HTML]{EFEFEF} 
\tool                 & \textbf{26.36}                               & \textbf{39.42}                               & \textbf{41.82}                               &                                              & 17.06                                        & \textbf{29.39}                               & \textbf{33.82}                               &                                              & 13.04                                        & \textbf{28.04}                               & \textbf{34.78}                               \\
w/ CF                 & XX                                           & XX                                           & XX                                           &                                              & XX                                           & XX                                           & XX                                           &                                              & XX                                           & XX                                           & XX                                           \\
\rowcolor[HTML]{EFEFEF} 
w/ CF+SQL             & XX                                           & XX                                           & XX                                           &                                              & XX                                           & XX                                           & XX                                           &                                              & XX                                           & XX                                           & XX                                           \\
w/ CF+Semantic        & XX                                           & XX                                           & XX                                           &                                              & XX                                           & XX                                           & XX                                           &                                              & XX                                           & XX                                           & XX                                           \\ \hline
\end{tabular}
